Subjective Databases

Online users are constantly seeking experiences, such as a hotel with clean rooms and a lively bar, or a restaurant for a romantic rendezvous. However, e-commerce search engines only support queries involving objective attributes such as location, price, and cuisine, and any experiential data is relegated to text reviews. In order to support experiential queries, a database system needs to model subjective data and also be able to process queries where the user can express varied subjective experiences in words chosen by the user, in addition to specifying predicates involving objective attributes. This paper introduces Opine, a subjective database system that addresses these challenges. We introduce a data model for subjective databases. We describe how Opine translates subjective queries against the subjective database schema, which is done by matching the user query phrases to the underlying schema. We also show how the experiential conditions specified by the user can be combined and the results aggregated and ranked. We demonstrate that subjective databases satisfy user needs more effectively and accurately than alternative techniques through experiments with real data of hotel and restaurant reviews.

==> interpreter.tex <==
\section{Subjective Query Interpreter} \label{sec:interpreter}


% \subsection{Extracting and aggregating subjective attributes}

% As mentioned in Section \ref{sec:model}, 

\subsection{Combining subjective query predicates with fuzzy logic}
\yuliang{moved the intro of fuzzy logic here. Will add more details later.}
Fuzzy logic \cite{klir1995fuzzy,fagin1996combining} provides a rigorous method of 
interpreting and combining multiple subjective query terms.
Intuitively, fuzzy logic generalizes propositional logic by considering 
truth values to be real numbers from $[0, 1]$ instead of 0 (False) or 1 (True).
Such generalization allows the reasoning of subjective predicates 
since the truth values are now representing the ``degrees of truth'' (e.g. the degree of quietness).
The standard logic operators (AND, OR and NOT) are also generalized.
For example, in a classic variant of fuzzy logic \cite{fagin1996combining}, 
AND$(x,y)$ is interpreted as MIN$(x,y)$, NOT$(x)$ is interpreted as $(1-x)$
and OR$(x,y)$ is interpreted as MAX$(x,y)$. \yuliang{Need to add more details depending on how much fuzzy logic we used in our techniques.}

\subsection{Interpretation}

Given a subjective SQL query $Q$, \system\ needs to translate $Q$ 
into a query $\tilde{Q}$ over the subjective database schema
so the query can be computed over the extracted and aggregated
subjective data. This is a challenging task because the natural language
query terms can be arbitrary text so the mapping from the query terms 
onto the subjective schema is not obvious. 
In addition, due to the subjectivity of the query, there is no unique standard way
of rewriting a query term. 
Multiple valid translations can be constructed according to multiple sources of
the knowledge about the query term, resulting in different quality of the
interpretation result and query performance. 
We summarize a list of sources that we consider in \system:
\begin{itemize}\parskip=0pt
\item \textbf{Word2Vec: } Word2vec enables computing the semantic distance
between any two words or phrases. For a given query term $q_i$, word2vec can be used
for finding the subjective attribute $A$ having linguistic variations and related entities
with shortest semantic distance with $q_i$. It is able to map simple query terms like 
``very clean room'' to the corresponding subjective attribute
\texttt{room\_cleanliness} very accurately, but it is less accurate 
for longer input. \yuliang{example needed}
\item \textbf{Co-occurrence: } Whether a query term $q_i$ is co-related to a subjective
attribute $A$ can also be measured by the the co-occurrence of $q_i$ and linguistic
variations of $A$ in a text corpus $T$. 
The data source of the subjective DB can be used as the text corpus $T$ 
and make an accurate interpretation only when the query term $q_i$ is a frequent term 
(e.g., ``honeymoon'') in the data source. Otherwise, a larger text corpus like the
open web needs to be considered. For example, the query term $q_i$ can be sent
to a web search engine (e.g., querying Google for ``honeymoon hotels'') 
and the correlated attributes can be extracted from the resulting web documents.
The cost of the latter case is likely to be more expensive as the search and the extraction needs to be performed online.
\item \textbf{Crowdsourcing: } Even when none of the above methods work, 
the interpreter can turn to crowdsourcing platforms like 
MTurk\footnote{\url{https://www.mturk.com/}} to obtain gold knowledge for interpreting 
the subjective query term. Depending on the money invested, the interpretation
task can be assigned to workers of different quality, resulting in
varying precision of the interpretation and response time.
Note that although realtime performance is unlikely,
the high precision of crowdsourcing might be desired by applications
like trip planning or hotel quality assurance analysis where
a fast response time is not a strict requirement.
\item \textbf{Cache: } Finally, if a query term has been correctly interpreted, 
the interpreter can cache the interpretation result and reuse in the future
at almost no cost.
\end{itemize}

We formulate the query interpretation with the above various knowledge sources
a \emph{multi-objective query optimization} problem.
Choosing between the different sources can be viewed as executing a query
with different strategies depending on the requirement of the applications.
We consider two competing objectives of the interpreter: 
(1) performance and (2) precision. In general, 
methods like word2vec yield faster running time but is less precise.
To the other extreme, crowdsourcing gives high precision but results in slow
query processing. 

We formulate the problem as the following. Each source of knowledge
is modeled as a \emph{rewriter}.
A rewriter $W$ translates $q_i$ into a predicate $W(q_i)$ 
over the attributes in the subjective schema.
For example, the co-occurrence rewriter $W^{\mathsf{CO}}$ rewrites
the input ``honeymoon'' into 
\begin{align*}
W^{\mathsf{CO}}(\text{``honeymoon''}) = \ & (room\_cleanliness.\text{``average'' } \mathbf{ and } \\
& bathroom.\text{``luxurious''}).
\end{align*}
In addition, each rewriter is associated with a time estimator $\mathtt{time}$
and a precision estimator $\mathtt{prec}$ both parameterized by the input query term.
The estimation can be made according to history of using the rewriter
or additional outputs like the distance score returned by the word2vec rewriter.
For example, we can have 
$\mathtt{time}^{\mathsf{w2v}}(\text{``honeymoon''}) = \text{ 10 ms}$ and
$\mathtt{prec}^{\mathsf{w2v}}(\text{``honeymoon''}) = 0.5$ 
for the word2vec rewriter on the input ``honeymoon''.

The optimization problem is formally defined as follows. Given a time budget 
$T_{max}$, we would like to choose a combination of rewriters for all query terms 
to maximize the average precision of the rewriting.
Namely, given a set of subjective query terms $\{q_1, \dots, q_n\}$ and
a set of rewriters $\{W_1, \dots, W_k\}$, find $b \in [k]^n$ (called the rewriter combination) that
\begin{equation} \label{equ:optimization}
\begin{array}{ll@{}ll}
\text{minimize}   & \displaystyle\dfrac{1}{n} \sum_{i=1}^n \mathtt{prec}^{W_{b_i}}(q_i)  \\
\text{subject to} & \displaystyle\sum_{i=1}^n \mathtt{time}^{W_{b_i}}(q_i) \leq T_{max}.
\end{array}
\end{equation}

The decision form of the above optimization problem is {\sc np-complete} by reduction from the 0/1 Knapsack problem \cite{knapsack}.

\begin{proof}
The decision form asks whether there exists rewriter combination $v \in [k]^n$ such that
the total running time is within the time budget $T_{max}$ and the average precision is above a precision threshold $P_{min}$.
Consider the following reduction from 0/1 Knapsack.
A knapsack instance states that given $n$ objectives ${1, \dots, n}$ where the $i$-th object has weight $w_i$ and value $v_i$.
Given a weight budget $W$ and minimal value $V$, decide whether there exists $u \in \{0,1\}^n$ such that
$\sum_{i=1}^n w_i u_i \leq W$ and $\sum_{i=1}^n v_i u_i > V$.

The reduction from 0/1 Knapsack constructs a list of $n$ query terms $\{q_1, \dots, q_n\}$
and two rewriters $\{W_0, W_1\}$ where $\mathtt{prec}^{W_0}(q_i) = \mathtt{time}^{W_0}(q_i) = 0$, 
$\mathtt{prec}^{W_1}(q_i) = n \cdot v_i$ and $\mathtt{time}^{W_1}(q_i) = w_i$. 
One can verify that there exists a solution to the 0/1 Knapsack problem iff
there exists a rewriter combination with total running time at most $W$ and average precision above $V$.
\end{proof}

\begin{theorem}\label{thm:npc}
Computing the optimal rewriting according to (\ref{equ:optimization}) is {\sc np-hard}.
\end{theorem}

\subsection{Computing the membership functions} \label{sec:mf}
For each subjective attribute $A$, a interpreted query term $q$ ($q$ is in the linguistic domain of $A$),
and a set $S$ of linguistic variations extracted from source data of an entity,
a membership function $mf(S, q)$ computes the degree of whether the entity satisfies the query condition $q$ given 
the set $S$ of extraction result.



%%% the following is an alternative defintion, but the algorithm is trivial if we consider one query term at a time 
%
% The optimization problem is associated with an objective function $M$
% over the overall estimated time and precision for the entire query.
% For simplicity, we consider $M$ a linear function
% over the total estimated time and the average precision.
% The optimization problem is formally defined as follows:
% Given a set of subjective query terms $\{q_1, \dots, q_n\}$ and
% a set of rewriters $\{W_1, \dots, W_k\}$, find
% $$ \argmax_{v \in [k]^n} \ \ c_1 \cdot \sum_{i=1}^n \mathtt{time}^{W_{v_i}}(q_i) +  
%                          c_2 \cdot \dfrac{1}{n} \sum_{i=1}^n \mathtt{prec}^{W_{v_i}}(q_i). 
% $$







% \yuliang{from alon's writeup.}
% \smallskip
% \noindent
% {\bf Handling linguistic variations in experiential attributes:} Some user queries express experiential attributes with synonyms of attributes in the schema, while others may only be related to existing attributes. For example, while the query {\sf extremely quiet} can be mapped to an existing attribute in the schema, the query {\sf romantic hotel} can only be mapped to the combination of {\sf excellent service} and {\sf luxurious bathrooms}.  \system\ includes a reformulation component that determines whether a user query can be expressed in terms of the schema. When the query is not fully supported by the existing schema, \system\ tries to answer it using data from the raw text of reviews and social media. 





% Major technical challenges:
% \begin{itemize}
% \item Schema construction
% \item Mapping from linguistic phrases to values (part of the data model right now)
% \item Aggregation: how do we allow the schema designer to define how each attribute is aggregated? 
% I think a declarative approach would work here. 
% We can show that most practically relevant use cases are expressible in the language.
% \item Crowd-Sensing: how do we construct the mapping from an arbitrary query to a query on the predefined schema?
% \item incremental query processing \yuliang{shall we do it in this paper? or defer it to the next one? :)}
% \end{itemize}

% Since there are several components that need to be tuned,
% it might make sense to provide some guidelines in strategies
% of tuning these parameters. There should be some metrics
% for evaluating effectiveness in each component,
% so the development process can be more modularized.

% \subsection{Subjective query interpreter}
% At query processing time, a query parser first translates the input query string into a set of objective and subjective predicates. 
% The objective predicates (e.g. \textsf{City = `Amsterdam'}) are evaluated directly on the objective data,
% but the subjective predicates (e.g. \textsf{<Romantic Hotel>})
% require further interpretation since they can be ambiguous or even not in the schema. 
% Such task requires external knowledge and reasoning to connect the predicates with the subjective schema.
% For example, interpreting the predicate \textsf{<Romantic Hotel>} requires the 
% knowledge that romantic hotel usually has stylish exterior and nice overlooking views from bedrooms. 
% Given such knowledge, \textsf{<Romantic Hotel>} can be rewritten into a conjunction
% $$\textsf{<stylish-exterior>} \land \textsf{<overlooking-view>}$$
% so that it can be evaluated on the aggregated subjective attributes
% of the entities.


% \yuliang{Next, we should talk about how to gather the knowledge to construct the ``crowd sense''.
% I think this is the most challenging task technically.}

% \yuliang{I think one potential solution is the following. 
% For each predicate X (e.g. romantic), we can perform a web search with query ``what are the most X hotel''. 
% The returned web documents seem to provide a lot information on what a hotel should have in order to be romantic.}


% \subsection{Processing the top-k, fuzzy logic queries}
% The interpreted query is of the 


% \subsection{Schema builder}
% The goal of this component is to help developer construct the subjective schema). For each attribute, the developer will provide the following:
% The entity names ("bedrooms", "bathrooms", "location", etc.)
% Example predicates. This can come in different forms, like "close to subway", ("quiet", "noisy"), "quiet room". And example scores assigned to each predicate. Like "quiet" : 0.6, "noisy" : 0.2

% What needs to be done:
% \begin{itemize}
% \item  Extend the set of predicates
% \item Assign scores to predicates
% \item Extract predicates from Text (this is the extractor)
% \end{itemize}

% \subsection{Aggregator}
% The goal of this component is to compute the aggregated views of the subjective attributes. The developer should be able to tune the aggregate function (beyond simple averaging). For example, the developer might want to assign different weight to different data sources (reviews vs. social media), to different dates (recent vs. old), to different review scores (1 star reviews are usually more important). The developer might also want to shift score based on user profiles (gender, nationality, avg review score, number of reviews given, etc.)

% The developer should also be able to quickly verify that the tuning is going to the right direction.
% \begin{enumerate}
%     \item \textbf{Hypothesis testing}: the developer should be able to whether a specific selection condition will significantly change the distribution of an attribute of the population (all data resources). This can be time vs. quietness, time vs. facilities (the hotel is renovated), etc. This can be done by performing hypothesis testing to see if the distribution is significantly different after the condition is applied (e.g. review\_year >= 2012). This step can also help the developer to construct reasonable reviews to show to the users.
%     \item \textbf{Weight assignment}: how to determine the weight of the different groups? i.e. different countries, different data sources, etc. How can the developer verify the effectiveness of the tuning?

% \end{enumerate}



% \subsection{Query Interpretor}
% Suppose that we want to use the web search results to help query interpretation. The goal is then to construct the predicate combination for any unseen predicate (assuming that we cached all seen predicates). Two cases can happen:
% 1. The predicate is an expression of a schema attribute (maybe "extrodinarily quiet"). For this case, we can simply map it to the closest predicate in the schema
% 2. The predicate is not of any schema attribute. For this case, we need to use the web search result. The result is a collection of HTML documents. From there, we need to extract paragraphs describing an entity that satisfies the query predicate. We can also extract entities in the DB that are mentioned in the search result. Then the set of extracted predicates of the entity can be used as the interpretation. The final output of the interpretation is a disjunction of conjunctions of predicates.

% For each single interpreted predicate, we still need to know how to compute a score of the predicate on each entity. Ideally, this function can also be tuned by the developer, but it is likely to be of the form of a sigmoid function. 

% \subsection{Experiment}
% Need to construct multiple sets of queries, more than one applications (we are building the hotel app, maybe we should build another one for restaurants, showing that our framework is general)

% \subsection{User interface design}
% Query interface, a scrolling control for tuning weights of different parameters

% \subsubsection{How do the user interact with the views?}
% Ideally, a query "is this hotel suitable for summer vacation?" can be answered by a view projecting the temperature attribute onto reviews created during the summer. The user might also want to interact by specifying further constraints like "only 1-star to 3-star reviews". This is related to query answering using views.

% Finally, we also need integration with elasticsearch.

